Iterative Algorithm for Discrete Structure Recovery

We propose a general modeling and algorithmic framework for discrete structure recovery that can be applied to a wide range of problems. Under this framework, we are able to study the recovery of clustering labels, ranks of players, signs of regression coefficients, cyclic shifts, and even group elements from a unified perspective. A simple iterative algorithm is proposed for discrete structure recovery, which generalizes methods including Lloyd's algorithm and the power method. A linear convergence result for the proposed algorithm is established in this paper under appropriate abstract conditions on stochastic errors and initialization. We illustrate our general theory by applying it on several representative problems: (1) clustering in Gaussian mixture model, (2) approximate ranking, (3) sign recovery in compressed sensing, (4) multireference alignment, and (5) group synchronization, and show that minimax rate is achieved in each case.

==> regression.tex <==
%!TEX root = manuscript20190725.tex

\newcommand{\tsnr}{\text{SNR}}
%\newcommand{\tslope}{\text{S\tslope}}


\subsection{Variable Sign Recovery with Hamming Loss}
In this section, we investigate the sign recovery problem of high dimensional regression. We assume 
\begin{align*}
Y = X\beta^* + w ,
\end{align*}
where $\{X_{i,j}\}_{1\in[n],j\in[p]},\{w_i\}_{i\in[n]}$ are i.i.d. $\mathcal{N}(0,1)$. Recall the definition of local statistics $T_j = \norm{X_j}^{-1}X_j^TY$, which can be simplified to
\begin{align*}
T_j = \mu_j (B^*,z^*_j) + \epsilon_j,
\end{align*}
where $\epsilon_j  =  \norm{X_j}^{-1}X_j^T w,\forall j\in[n]$ which satisfies $\epsilon_j|X \sim \mathcal{N}(0,1)$, and
\begin{align*}
\mu_j(B^*,z^*_j) = \norm{X_j} \beta_j^* +  \norm{X_j} ^{-1} \sum_{l\in[p]\setminus\cbr{j}} \beta_l^* X_j^T X_l.
\end{align*}
Recall the definition of $t(X_j)$:
\begin{align}
t(X_j)=\frac{\lambda}{2}+\frac{\log\frac{p-s}{s}}{\lambda\|X_j\|^2} \label{eqn:reg_t}.
\end{align}
Applying Algorithm \ref{alg:general} to this problem, we can write the iterations as
\begin{align*}
z_j^{(t)} &= \begin{cases}
1, & \frac{1}{\|X_j\|^2}\br{X_j^TY-\sum_{l\in[p]\backslash\{j\}}\hat \beta_l (z^{(t-1)})X_j^TX_l} > t(X_j), \\
0, & -t(X_j) \leq  \frac{1}{\|X_j\|^2}\br{X_j^TY-\sum_{l\in[p]\backslash\{j\}}\hat \beta_l (z^{(t-1)})X_j^TX_l} \leq t(X_j), \\
-1, & \frac{1}{\|X_j\|^2}\br{X_j^TY-\sum_{l\in[p]\backslash\{j\}}\hat \beta_l (z^{(t-1)})X_j^TX_l} < -t(X_j),
\end{cases}
\end{align*}
where
\begin{align}
\hat \beta (z) &= \argmin_{\left\{\beta\in\mathbb{R}^p: \beta_j=\beta_j|z_j|\right\}}\|y-X\beta\|^2.\label{eq:beta-z-reg}
\end{align}


Now we  are going to apply our general convergence analysis in Section \ref{sec:con} to this case. By Equation (\ref{eqn:reg_mu_a_def}), we have
\begin{align}
\norm{\mu_j(B^*,z^*_j)  -\mu_j(B^*,b) }^2 = \begin{cases}
\lambda^2\|X_j\|^2, &  z^*_j=0, b = \pm 1\\
|\beta_j^*|^2\|X_j\|^2, &z^*_j=\pm 1, b=0\\
4|\beta_j^*|^2\|X_j\|^2, &  z^*_j=\pm 1, b =\mp 1
\end{cases}\label{eqn:reg_mu_diff}
\end{align}
which leads to  the  loss function as:
\begin{align}
\ell(z,z^*)=\sum_{j=1}^p\left(\lambda^2\|X_j\|^2\indc{z_j^*=0,z_j\neq 0}+|\beta_j^*|^2\|X_j\|^2\indc{z_j^*\neq 0,z_j=0}+4|\beta_j^*|^2\|X_j\|^2\indc{z_jz_j^*=-1}\right).\label{eqn:reg_l}
\end{align}


Note that $\mu_j(B^*,a)\neq \nu_j(B^*,a)$ in this case. By Equation (\ref{eqn:reg_mu_a_def}) and Equation (\ref{eqn:reg_nu_a_def}), we have the explicit formulas for $\Delta_j(z_j^*,b)^2$ as follows
\begin{align}
\Delta_j(z_j^*,b)^2 = 
\begin{cases}
 4t(X_j)^2 \|X_j\|^2 , & z_j^*=0,b=\pm 1 \\
4 t(X_j) (|\beta_j^*| - t(X_j))\|X_j\|^2, & z_j^*=\pm 1, b=0\\
 8|\beta_j^*| t(X_j)\|X_j\|^2, & z_j^*=\pm 1, b=\mp 1.
\end{cases}\label{eqn:reg_delta}
\end{align}
Note that at this moment, $\Delta_j(z_j^*,b)^2$ define above might be negative, as $|\beta_j^*| - t(X_j)$ may be negative. However, after we establish some condition on the minimal signal strength (i.e., Equation (\ref{eqn:lambda_def})), we will show such scenario is very unlikely. That is, we will later show with high probability $\Delta_j(z_j^*,b)^2>0$ for all $b\neq z^*_j$ and $j\in[p]$.

%$$\epsilon_j=\frac{X_j^Tw}{\|X_j\|}.$$

Due to the fact that 
\begin{align*}
&\nu_j(\wh{B}(z),a)-\nu_j(B^*,a)-\nu_j(\wh{B}(z),b)+\nu_j(B^*,b)=0\\
& \nu_j(\wh{B}(z^*),a)-\nu_j(\wh{B}(z),a)-\nu_j(\wh{B}(z^*),b)+\nu_j(\wh{B}(z),b)=0
\end{align*}
for all $a,b\in\{0,1,-1\}$, we have
\begin{align*}
&F_j(a,b;z)=0 \\
& G_j(a,b;z)=0 
\end{align*}
The only error terms left to be controled turns out to be
\begin{align*}
& H_j(a,b;z)=2(a-b)\|X_j\|t(X_j)\left(\|X_j\|^{-1}\sum_{l\in[p]\backslash\{j\}}\wh{\beta}_l(z)X_j^TX_l-\|X_j\|^{-1}\sum_{l\in[p]\backslash\{j\}}\beta_l^*X_j^TX_l\right).
\end{align*}
Decompose it into
\begin{align*}
& H'_{i}(a,b;z) =  \iprod{\nu_i (B^*,a)-\nu_i (B^*,b)}{\nu_i (\wh{B}(z^*),b)-\nu_i (B^*,b)} \\ 
\text{and } & H''_{i}(a,b;z) =  \iprod{\nu_i (B^*,a)-\nu_i (B^*,b)}{\nu_i (\wh{B}(z),b)-\nu_i (\wh{B}(z^*),b)}.
\end{align*}

\begin{lemma}\label{lem:reg-error}
Under the assumption that  $s\log p \leq n$ %and $\lim_{p\rightarrow\infty}s/p <1/2$ hold
holds, for any constants $C_0,C'>0$, there exists a constant $C>0$ that only depends on $C_0,C'$, such that
 %\nb{note that $H'$ is invariant to $z$}
\begin{align}\label{eqn:reg_H_p}
\max_{z:\ell(z,z^*)\leq C_0sn\lambda^2}\max_{b\in\cbr{0,1,-1} }\max_{i\in[p]}\abs{\frac{H'_{i}(z_i^*,b;z)}{\Delta_i(z_i^*,b)^2}} & \leq  \sqrt{\frac{4Cs\log^2 p}{n}}  \frac{1}{\min_{i\in[p]}\sqrt{n}\abs{\abs{\beta_i^*} -  t(X_i)}},
\end{align}
and
\begin{align}\label{eqn:reg_H_pp}
&\max_{z:\ell(z,z^*)\leq C_0sn\lambda^2}\max_{b\in\cbr{0,1,-1}}\max_{T\in[p]} \frac{1}{s+\abs{T}}  \sum_{i\in T}  \frac{H_i''(z_i^*,b;z)^2\|\mu_j(B^*,b)-\mu_j(B^*,z_i^*)\|^2}{\Delta_i(z_i^*,b)^4\ell(z,z^*)} \nonumber  \\
&\leq C\br{\frac{\log^2 p}{n} + \frac{\log^2 p}{\lambda^2n^2}}\max_{i\in[n]}\max\cbr{4\br{\frac{\abs{\beta^*_i}}{\abs{\beta^*_i} - t(X_i)}}^2,\br{\frac{\lambda}{t(X_i)}}^2},
\end{align}
hold with probability at least $1-p^{-C'}$.
\end{lemma}

To make the Condition ? hold, we need assumption on the minimum signal strength. First we define $\tsnr$ (i.e., signal-to-noise) as follows,
\begin{align}\label{eqn:reg_snr_def}
\tsnr \triangleq \frac{\lambda \sqrt{n}}{2} - \frac{\log \frac{p-s}{s}}{\lambda \sqrt{n}}.
\end{align}
As we will later see in Theorem \ref{thm:reg-main} and Proposition \ref{prop:reg_minimax_lower}, it plays the exact same role as $\Delta_{\min}$ in Section 4.1 and $\sqrt{p\beta^{*2}}$ in Section 4.2.
We assume $\lambda$ satisfies the following condition:
%Equation (\ref{eqn:reg_H_pp}) implies that  when we further assume $s\log^4 p =o(n)$ and the signal strength $\lambda$ satisfies
\begin{align}\label{eqn:lambda_def}
\tsnr \rightarrow\infty.
\end{align}
%We  as it turns out to be the signal-to-noise ratio for this problem, which . 
%which as we will show later, turns out to  for the minimax rate.

In Lemma \ref{lem:random-events-reg}, we have $\abs{\norm{X_j} - n}\leq C\sqrt{n\log p}$ for all $j\in[n]$ with high probability. Proved in Lemma \ref{lem:lambda_diff} , Equation (\ref{eqn:lambda_def}) helps to characterize the following quantities:
\begin{itemize}
\item $\Delta_j(z_j^*,b)^2 > 0,\forall b\neq z^*_j,j\in[p]$
\item $\sqrt{n}\br{\abs{\beta_i^*} - t(X_j)}\rightarrow\infty , \forall j \in[p]$
\item $\frac{\abs{\beta^*_j}}{\abs{\beta^*_j} - t(X_i)} \leq \sqrt{\log p},\forall j\in[p]$
\item $\lambda \geq t(X_j),\forall j\in[p]$ and $n\lambda^2\geq 1$.
\end{itemize}
These make both of the right hand sides of Equation (\ref{eqn:reg_H_p}) and Equation (\ref{eqn:reg_H_pp}) to $o(1/\log p)$, as we state in following corollary.

\begin{corollary}\label{cor:reg-error}
Assume  $ s\log^4 p =o(n)$,  $\lim_{p\rightarrow\infty}s/p <1/2$, and $\tsnr\rightarrow\infty$. For any constant $C_0 >0$, we have
\begin{align*}
\max_{z:\ell(z,z^*)\leq C_0sn\lambda^2}\max_{b\in\cbr{0,1,-1} }\max_{i\in[p]}\abs{\frac{H'_{i}(z_i^*,b;z)}{\Delta_i(z_i^*,b)^2}} =o\br{\frac{1}{\log p}}
\end{align*}
and
\begin{align*}
\max_{z:\ell(z,z^*)\leq C_0sn\lambda^2}\max_{b\in\cbr{0,1,-1}}\max_{T\in[p]} \frac{1}{s+\abs{T}}  \sum_{i\in T}  \frac{H_i''(z_i^*,b;z)^2\|\mu_j(B^*,b)-\mu_j(B^*,z_i^*)\|^2}{\Delta_i(z_i^*,b)^4\ell(z,z^*)}  =o\br{\frac{1}{\log p}},
\end{align*}
hold with probability at least $1-p^{-C}$ for some constant $C>0$.
\end{corollary}


Next, we are going to establish some upper bound on $\xi_{\rm ideal}(\delta)$ in Condition ?. Before that, we define 
\begin{align}\label{eqn:psi_def}
\psi(n,p,s,\lambda,\delta,C)= & s\pbr{\frac{\epsilon}{1-\delta} \geq \norm{\zeta} \br{\lambda - t(\zeta)}\;\&\; \abs{\norm{\zeta} -n}\leq C\sqrt{n\log p}} \nonumber \\
&\quad+ \br{p-s}\pbr{\frac{\epsilon}{1-\delta} \geq \norm{\zeta}t(\zeta)\;\&\; \abs{\norm{\zeta} -n}\leq C\sqrt{n\log p}},
\end{align}
where $\epsilon\sim\mathn(0,1)$ and $\zeta\sim\mathn(0,I_n)$ and they are independent of each other.

\begin{lemma}\label{lem:reg-ideal}
Assume $s\log p\leq n$, $\lim_{p\rightarrow\infty}s/p <1/2$, and $\tsnr\rightarrow\infty$. For any $w\rightarrow\infty$, any $\delta =o(1)$, any constant $C'>0$, there exists a constant $C>0$ that only depends on $C'$, such that 
\begin{align*}
\xi_{\rm ideal}(\delta) \leq 16wn  \lambda^2\psi(n,p,s,\lambda,\delta,C),
\end{align*}
with probability at least $1-w^{-1} - p^{-C'}$.
\end{lemma}

We need to have some extra constraint on $w$ to make sure $\xi_{\rm ideal}(\delta)$ is relative small so that the Condition E can be guaranteed. On top of the assumptions stated in Lemma \ref{lem:reg-ideal}, if we further assume $\delta =o((\log p)^{-1})$, we have $\psi(n,p,s,\lambda,\delta,C) \leq \psi(n,p,s,\lambda,(\log p)^{-1},0)$. By Proposition \ref{prop:reg_rate_simplify}, it turns out that $\psi(n,p,s,\lambda,(\log p)^{-1},0) =o(s)$. As a result, to have Condition E guaranteed, it is sufficient to have $w\rightarrow\infty$ but $w\psi(n,p,s,\lambda,(\log p)^{-1},0) =o(s)$.

%which turns out to be $o(s)$ by , under the ass
%
%Proposition \ref{prop:reg_rate_simplify} gives an explicit formula of $\psi(n,p,s,\lambda,\delta,C)$, showing that $\psi(n,p,s,\lambda,\delta,C) =o(s)$ assuming $\delta =o(1/\log p)$, in additional to the assumptions stated in Lemma \ref{lem:reg-ideal}. This indicates we can choose some $w\rightarrow\infty$ wisely, such that $\xi_{\rm ideal}(\delta) =o\br{sn\lambda^2}$, small so that the Condition E can be satisfied. Note that $\psi(n,p,s,\lambda,\delta,C) \leq \psi(n,p,s,\lambda,1/\log p,0)$ which is also $o(s)$
%. 

With the help of Lemma \ref{lem:rank-error} and Lemma \ref{lem:ranking-ideal}, we can specialize Theorem \ref{thm:main-simple} into the following result.


%\begin{align*}
%\E \xi_{\rm ideal}(\delta) & \leq 8 \sum_{j\in S^*}\abs{\beta^*_j}^2 \pbr{\epsilon_j \leq -\br{1-\delta} \norm{X_j}\br{\abs{\beta_j^*}  - t(X_j)}} + 8 \sum_{j\notin S^*}\lambda^2 \pbr{\epsilon_j \leq -\br{1-\delta} \norm{X_j} t(X_j)} \\
%& =  8 \sum_{j\in S^*}\abs{\beta^*_j}^2 \pbr{\frac{\epsilon_j}{ {1-\delta}} \geq \norm{X_j}\br{\abs{\beta_j^*}  - t(X_j)}} + 8 \sum_{j\notin S^*}\lambda^2 \pbr{\frac{\epsilon_j}{ {1-\delta}} \geq  \norm{X_j} t(X_j)}.
%\end{align*}
%
%
%Define a quantity
%\begin{align*}
%\psi(n,p,s,\lambda,\delta)= s\pbr{\frac{\epsilon}{1-\delta} \geq \norm{\zeta} \br{\lambda - t(\zeta)}} + \br{p-s}\pbr{\frac{\epsilon}{1-\delta} \geq \norm{\zeta}t(\zeta)},
%\end{align*}
%where $\epsilon\sim\mathn(0,1)$ and $\zeta\sim\mathn(0,I_n)$ and they are independent of each other.
%
%Now we are going to show the function $f(y) = y^2\pbr{\frac{\epsilon}{1-\delta} \geq \norm{\zeta} \br{y - t(\zeta)}}$ is a decreasing function of $y$ when $y\geq \lambda$ and $\lambda >0$. To establish to this, first we have 
%\begin{align*}
%f(y) = y^2\pbr{\frac{\epsilon}{1-\delta} \geq \norm{\zeta} \br{\br{y -\frac{\lambda}{2}} - \frac{\log \frac{p-s}{s}}{\lambda \norm{\zeta}^2} }} = y^2 \int p(u) \int^\infty_{\br{1-\delta} u \br{\br{y -\frac{\lambda}{2}} - \frac{\log \frac{p-s}{s}}{\lambda u^2 } }} \frac{1}{\sqrt{2\pi}}\ebr{-\frac{v^2}{2}} dvdu,
%\end{align*}
%where $p(\cdot)$ is the density of $\norm{\zeta}$. Then we have
%\begin{align*}
%f'(y) &= \int p(u) \br{2y  \int^\infty_{\br{1-\delta} u \br{\br{y -\frac{\lambda}{2}} - \frac{\log \frac{p-s}{s}}{\lambda u^2 } }} \frac{1}{\sqrt{2\pi}}\ebr{-\frac{v^2}{2}} dv   - y^2\frac{\br{1-\delta}u}{\sqrt{2\pi}}\ebr{-\frac{\br{\br{1-\delta} u \br{\br{y -\frac{\lambda}{2}} - \frac{\log \frac{p-s}{s}}{\lambda u^2 }}}^2}{2}}  }\\
%& \leq \int p(u) \frac{y}{\sqrt{2\pi}}\br{\frac{2}{\br{1-\delta} u \br{\br{y -\frac{\lambda}{2}} - \frac{\log \frac{p-s}{s}}{\lambda u^2 } }} -y\br{1-\delta}u}\ebr{-\frac{\br{\br{1-\delta} u \br{\br{y -\frac{\lambda}{2}} - \frac{\log \frac{p-s}{s}}{\lambda u^2 }}}^2}{2}}  du.
%\end{align*}





\begin{thm}\label{thm:reg-main}
Assume  $s\log^4 p =o(n)$, $\lim_{p\rightarrow\infty}s/p <1/2$, and $\tsnr\rightarrow\infty$. Suppose $z^{(0)}$ satisfies $\ell(z^{(0)},z^*)\leq C_0n\lambda^2$ with probability at least $1-\eta$ for some constant $C_0>0$. Then we have for any $w\rightarrow \infty$ with $w\psi(n,p,s,\lambda,(\log p)^{-1},0) =o(s)$, and any constant $C'>0$, there exists some $\delta=o(1/\log p)$, and  a constant $C>0$ that only depends on $C_0,C'$, such that
\begin{align*}
\ell(z^{(t)},z^*) \leq 16wn  \lambda^2 \psi(n,p,s,\lambda,\delta,C) + \frac{1}{2}\ell(z^{(t-1)},z^*)\quad \forall t\geq 1,
\end{align*}
with probability at least $1-\eta - w^{-1}- p^{-C'}$.
\end{thm}

%Using Equation (\ref{eqn:reg_h}) for the  relation between $\ell(z,z^*)$ and $h(z,z^*)$, immediately we obtain upper bound on the Hamming loss $h(z,z^*)$. However, we state in  the following corollary, in term of the normalized Hamming distance
We define the normalized Hamming distance between $z,z^*$ as follows.
\begin{align*}
H(z,z^*)  = \frac{1}{s} \sum_{j=1}^p \indc{z_j \neq z^*_j},
\end{align*}
which is more natural measurement for the distance between $z$ and $z^*$, in the context of sign recovery.
%which is consistent with the losses $\misc(\cdot, \cdot)$ and $L_2(\cdot, \cdot)$ used in the previous two cases. 
It is obvious that we have 
\begin{align*}
H(z,z^*)   \leq \frac{\ell(z,z^*)}{s\lambda^2\min_j \norm{X_j}^2} \leq \frac{2\ell(z,z^*)}{sn\lambda^2},
\end{align*}
where the last inequality is valid when Equation (\ref{eqn:re0}) holds.

\begin{corollary}\label{cor:reg-main-h}
Assume  $s\log^4 p =o(n)$, $\lim_{p\rightarrow\infty}s/p <1/2$, and $\tsnr\rightarrow\infty$. Suppose $z^{(0)}$ satisfies $\ell(z^{(0)},z^*)\leq C_0n\lambda^2$ with probability at least $1-\eta$ for some constant $C_0>0$. Then we have for any $w\rightarrow \infty$ with $w\psi(n,p,s,\lambda,(\log p)^{-1},0) =o(s)$, and any constant $C'>0$, there exists some $\delta=o(1/\log p)$, and  a constant $C>0$ that only depends on $C_0,C'$, such that
\begin{align}\label{eqn:reg-main-h-bound}
H(z^{(t)},z^*) \leq 32ws^{-1}\psi(n,p,s,\lambda,\delta,C) + 2^{-t} \quad \text{for all }t\geq 1
\end{align}
with probability at least $1-\eta - w^{-1}-p^{-C'}$.
\end{corollary}



Proposition \ref{prop:reg_rate_simplify} gives an simple and explicit upper bound for $\psi'$. Recall the definition of $\tsnr$ as in Equation (\ref{eqn:reg_snr_def}). By taking $w = \ebr{ \tsnr }$, Corollary \ref{cor:reg-main-h} implies the following.

%We can further give an explicit expression. By Proposition \ref{prop:reg_rate_simplify}, we can take , and it gives us the following result.

\begin{corollary}\label{eqn:reg-main-h-bound-2}
Assume  $s\log^4 p =o(n)$, $\lim_{p\rightarrow\infty}s/p <1/2$, and $\tsnr\rightarrow\infty$. Suppose $z^{(0)}$ satisfies $\ell(z^{(0)},z^*)\leq C_0sn\lambda^2$ with probability at least $1-\eta$ for some constant $C_0>0$. Then we have 
\begin{align*}
H(z^{(t)},z^*) \leq \ebr{- \frac{\br{1+o(1)}\tsnr^2}{2}} +2^{-t}  \quad \text{for all }t\geq 1,
\end{align*}
with probability at least $1-\eta - \ebr{- \tsnr} -p^{-C}$ for some constant $C>0$.
\end{corollary}

Since $H(z,z^*) $ takes values in the set $\cbr{j/s:j\in[p]\cup[0]}$, the term $2^{-t}$ in Equation (\ref{eqn:reg-main-h-bound}) is negligible as long as $2^{-t} =o(p^{-1})$. We therefore can claim with high probability,
\begin{align}\label{eqn:reg_final_rate}
H(z^{(t)},z^*) \leq  \ebr{- \frac{\br{1+o(1)}\tsnr^2}{2}}\quad \text{for all }t\geq 3\log p.
\end{align}

The minimax lower bound is given in Theorem 2.1 of \citep{ndaoud2018optimal}. After some simplification, it leads to the following  Proposition \ref{prop:reg_minimax_lower}.
\begin{proposition}\label{prop:reg_minimax_lower}
Assume $s\log p \leq n$, $\lim_{p\rightarrow\infty}s/p <1/2$,  and $\tsnr\rightarrow\infty$, we have 
\begin{align*}
\inf_{\hat z}\sup_{\beta \in B_{s,\lambda}} \E H(\hat z,z^*) \geq \ebr{- \frac{\br{1+o(1)} \tsnr^2}{2}} - 2\ebr{-\frac{s}{8}},
\end{align*}
where $B_{s,\lambda}=\cbr{\beta\in\mathr^p:\norm{\beta}_0 \leq s, \abs{\beta_j} \geq \lambda,\forall j\in[p] \text{ s.t. }\beta_j\neq 0}$.
If $\tsnr$ does not go to infinity, we have $\inf_{\hat z}\sup_{\beta \in B_{s,\lambda}} \E H(\hat z,z^*) \geq c$ for some constant $c>0$.
\end{proposition}

Together with Equation (\ref{eqn:reg_final_rate}), Proposition \ref{prop:reg_minimax_lower} shows that $\tsnr\rightarrow\infty$ is the sufficient and  necessary condition to have consistence support recovery, in the sense that $ H(\hat z,z^*) \rightarrow\infty$. There are two terms in Proposition \ref{prop:reg_minimax_lower}. The second term $2\ebr{-\frac{s}{8}}$ is secondary, if not negligible, compared to the first term. Note that $ 2\ebr{-s/8} < s^{-1}$ when  $s\geq 40$, and recall that $H(z,z^*) $ takes values in the set $\cbr{j/s:j\in[p]\cup[0]}$. This makes the first term $\ebr{- \br{1+o(1)} \tsnr^2/2}$ the main term for the minimax lower bound for support recovery. As it matches with Equation (\ref{eqn:reg_final_rate}), we come to the conclusion that $H(z^{(t)},z^*) $ achieves the minimax rate after $t\geq 3\log p$ iterations.

The upper bound we establish above is comparable to \citep{ndaoud2018optimal}. Corollary \ref{cor:reg-main-h} implies our iterative  algorithm essentially achieves $\psi(n,p,s,\lambda,\delta,C)$; while in Theorem 2.2 of \citep{ndaoud2018optimal}, the performance of their algorithm is upper bounded by some quantity very similar to $\psi(n,p,s,\lambda,\delta,C)$. Despite some subtle difference, they are close to each other. As we mention earlier, the key difference between our result and \citep{ndaoud2018optimal} is that we implement our algorithm on the same dataset and are able to analysis it, but in \citep{ndaoud2018optimal} they need sample splitting to have   independent samples for different steps.

 %the theoretical guarantee they provide for  . , the two results are similar to each other, in terms of form. However, 


%It is established , that the  minimax lower bound for $H(\cdot, \cdot )$ loss is  $\frac{s^{-1}}{2}\psi(n,p,s,\lambda) - 2\ebr{-s/8}$. Note that $ 2s\ebr{-s/8} \leq 1$ is negligible when $s\geq 40$. The main term $\frac{s^{-1}}{2}\psi(n,p,s,\lambda)$ can be simplified according to Proposition \ref{prop:reg_rate_simplify}. This shows that the minimax lower bound also takes the form $\ebr{- \frac{1+o(1)}{2}\tsnr^2}$. As a consequence, $H(z^{(t)},z^*)$ achieves the minimax rate.




To close this section, we discuss how to initialize our iterative algorithm  for sign recovery. Our initialization procedure is defined as follows, utilizing the Square-Root SLOPE \citep{derumigny2018improved, ndaoud2018optimal}:
\begin{enumerate}
\item Compute the  Square-Root SLOPE estimator $\tilde \beta$. That is,
\begin{align*}
\tilde \beta= \argmin_{\beta\in\mathr^p} \br{n^{-\frac{1}{2}}\norm{Y - X\beta} + 2\abs{\beta}_* },
\end{align*}
where $\abs{\beta}_* = \sum_{j=1}^p\lambda_j \beta^*_j$ with $\lambda_j = A \sqrt{n^{-1}\log \br{2pj^{-1}}}$ for all $j\in[p]$ and $\beta \in\mathr^p$ with some sufficiently large constant $A>0$.
\item Compute $\tilde z \in\cbr{1,0,-1}^p$ by
\begin{align*}
\tilde z_j =  \text{sign}\br{\tilde \beta_j} \indc{\abs{\tilde \beta_j} \geq \frac{\lambda}{2}},\forall j\in[p].
\end{align*}
\end{enumerate}
The following proposition characterizes the theoretical performance of $\tilde z$. It guarantees $\tilde z$ can be used as an initializer $\hat z^{(0)}$ in our Theorem \ref{thm:reg-main}, Corollary \ref{cor:reg-main-h} and Corollary \ref{eqn:reg-main-h-bound-2}.
\begin{proposition}\label{prop:reg_init}
Assume $s\log p \leq n$, $\lim_{p\rightarrow\infty}s/p <1/2$,  and $\tsnr\rightarrow\infty$. For some sufficiently large $A >0$, there exists constants $C_0,C'>0$, such that 
\begin{align*}
\ell(\tilde z, z^*) \leq C_0sn\lambda^2
\end{align*}
with probability at least $1 - 2^{-C' s} - p^{-C'}$.
\end{proposition}



%\begin{align*}
%\psi'(n,p,s,\lambda,\delta,C) &\leq    s \pbr{\frac{\epsilon}{1-\delta} \geq u_{\min}\br{\frac{\lambda}{2} - \frac{\log \frac{p-s}{s}}{\lambda u_{\min}^2}} }  + \br{p-s}\pbr{\frac{\epsilon}{1-\delta} \geq  \sqrt{2\log \frac{p-s}{s}}}\\
%& \leq \frac{s}{\sqrt{2\pi} \br{1-\delta} u_{\min}\br{\frac{\lambda}{2} - \frac{\log \frac{p-s}{s}}{\lambda u_{\min}^2}}} \ebr{- \frac{\br{ \br{1-\delta} u_{\min}\br{\frac{\lambda}{2} - \frac{\log \frac{p-s}{s}}{\lambda u_{\min}^2}}}^2}{2}}\\
%&\quad + \frac{p-s}{\sqrt{2\pi} \br{1-\delta} \sqrt{2\log \frac{p-s}{s}}} \ebr{- \frac{2\log \frac{•}{•}}{•}}
%\end{align*}





%\begin{align*}
%\max_{\{z:\ell(z,z^*)\leq\tau\}}\sum_{j=1}^p\max_{b\in\cbr{0,1,-1}\backslash\{z_j^*\}}\frac{H_j(z_j^*,b;z)^2\|\mu_j(B^*,b)-\mu_j(B^*,z_j^*)\|^2}{\Delta_j(z_j^*,b)^4\ell(z,z^*)} \leq ,
%\end{align*}







